PerLA: Perceptive 3D Language Assistant

Enabling Large Language Models (LLMs) to understand the 3D physical world is an emerging yet challenging research direction. Current strategies for processing point clouds typically downsample the scene or divide it into smaller parts for separate analysis. However, both approaches risk losing key local details or global contextual information. In this paper, we introduce PerLA, a 3D language assistant designed to be more perceptive to both details and context, making visual representations more informative for the LLM. PerLA captures high-resolution (local) details in parallel from different point cloud areas and integrates them with (global) context obtained from a lower-resolution whole point cloud. We present a novel algorithm that preserves point cloud locality through the Hilbert curve and effectively aggregates local-to-global information via cross-attention and a graph neural network. Lastly, we introduce a novel loss for local representation consensus to promote training stability. PerLA outperforms state-of-the-art 3D language assistants, with gains of up to +1.34 CiDEr on ScanQA for question answering, and +4.22 on ScanRefer and +3.88 on Nr3D for dense captioning. https://gfmei.github.io/PerLA/

==> main/sections/copy.tex <==
% Specifically, we introduce a differentiable MinCut clustering algorithm specifically designed to reduce high computational costs. Instead of relocating every point in the point cloud, we shift a selected group of predetermined anchors.

% %-------------------------------------
% \begin{equation}\label{eq:graph}
%     \mathcal{W}_{ij} = 
%     \begin{cases}
%         \frac{\bm{f}_i^\top \bm{f}_j}{\|\bm{f}_i\| \|\bm{f}_j\|} + 1, & \text{if } \|p_i - p_j\| < r, \\
%         0, & \text{otherwise}.
%     \end{cases}
% \end{equation}
% %-------------------------------------

% The cluster centroids for positions and features are represented by $\bar{\bm{P}} = \{\bar{\bm{p}}_j\}$ and $\bar{\bm{F}} = \{\bar{\bm{f}}_j\}$, respectively, calculated as:
% %-------------------------------------
% \begin{equation} \label{eq:center}
% \begin{aligned}
%     \bar{\bm{p}}_j &= \frac{1}{\sum_{i=1}^{N} s_{ij}} \sum_{i=1}^{N} s_{ij} \bm{p}_i, \\
%     \bar{\bm{f}}_j &= \frac{1}{\sum_{i=1}^{N} s_{ij}} \sum_{i=1}^{N} s_{ij} \bm{f}_i.
% \end{aligned}
% \end{equation}
% %-------------------------------------
% Then, $\bar{\bm{P}}$ and $\bar{\bm{F}}$ are considered as the object centroids and their corresponding feature representations.
\paragraph{Min-cut loss.}
The clustering is optimized using the normalized cut relaxation proposed in \cite{bianchi2020spectral}. The loss function for the normalized cut is defined as:
%-------------------------------------
\begin{equation}
    \mathcal{L}_{\text{NCut}} = 1 - \frac{\text{Tr}(S^T \mathcal{W} S)}{\text{Tr}(S^T \mathcal{D} S)} + \left\| \frac{S^T S}{\|S^T S\|_F} - \frac{I_K}{\sqrt{K}} \right\|_F,
\end{equation}
%-------------------------------------
The parameter $K$ represents the number of disjoint sets we aim to partition the point cloud into, and $I_K$ is the identity matrix.

\paragraph{Reconstruction loss.}
Based on the cluster centroids and the cluster assignment matrix, the points can be reconstructed as follows:
%-------------------------------------
\begin{equation} \label{eq:reconstruction}
    \begin{aligned}
        \hat{\bm{p}}_i &= \frac{1}{\sum_{j=1}^{K} s_{ij}} \sum_{j=1}^{K} s_{ij}\cdot \text{stop}\left(\bar{\bm{p}}_j\right), \\
        \hat{\bm{f}}_i &= \frac{1}{\sum_{j=1}^{K} s_{ij}} \sum_{j=1}^{K} s_{ij} \cdot\text{stop}\left(\bar{\bm{f}}_j\right),
    \end{aligned}
\end{equation}
where $\text{stop}(\cdot)$ denotes stopping the gradient.


We apply a one-layer Graph Convolutional Network (GCN) on the graph $\mathcal{G}^g$ to obtain an updated feature matrix $\hat{\mathcal{F}}^g$. Let $S$ be the output of a Multi-Layer Perceptron (MLP) with a softmax function applied to $\mathcal{F}_G$:
%-------------------------------------
\begin{equation}
    \begin{aligned}
        {\mathcal{F}}^G &= \text{GCN}\left(\hat{\mathcal{F}}^g, \mathcal{W}^g; \Theta_{\text{GCN}}\right), \\
        S &= \text{MLP}\left(\mathcal{F}^G; \Theta_{\text{MLP}}\right),
    \end{aligned}
\end{equation}
%-------------------------------------
where $\Theta_{\text{GCN}}$ and $\Theta_{\text{MLP}}$ are trainable parameters. The GNN output $S$ represents the cluster assignment matrix, containing vectors that indicate the probability of each point belonging to a particular cluster.

==> main/tables/ab_ab_gcn.tex <==
% We conducted the GCN ablation and reported the results in the table below. 
% The introduction of GCN consistently improves the performance across three datasets, confirming its effectiveness.
% We will add this analysis in the revision of the paper.
%+++++++++++++++++++++++++++++++++++++++++++++++++++++
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{0.5}
    \tabcolsep 5pt
    \vspace{-3mm}
    \resizebox{1\columnwidth}{!}{%
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{4}{c|}{ScanQA} & \multicolumn{4}{c|}{ScanRefer@0.5} & \multicolumn{4}{c}{Nr3D@0.5} \\
 & C$\uparrow$ & B4$\uparrow$ & M$\uparrow$ & R$\uparrow$ & C$\uparrow$ & B4$\uparrow$ & M$\uparrow$ & R$\uparrow$ & C$\uparrow$ & B4$\uparrow$ & M$\uparrow$ & R$\uparrow$ \\ 
        \midrule
        w/o GCN & {77.6} & {13.9} & {15.9} & {39.3} & {69.0} & {37.4} & 28.7 & {55.6} & {54.3} & {29.8} & {27.4} & {58.3}\\ 
        \rowcolor{lightgreen}w/GCN  & \bf78.1 & \bf14.5 & \bf17.4 & \bf39.6 & \bf69.4 & \bf38.0 & \bf29.1 &  \bf56.8 & \bf55.1 & \bf31.2 & \bf28.5 & \bf59.1 \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
\end{table}
%+++++++++++++++++++++++++++++++++++++++++++++++++++++
